AndroCon: Conning Location Services in Android

Mobile device hackers often target ambient sensing, human activity identification, and interior floor mapping. In addition to overt signals like microphones and cameras, covert channels like WiFi, Bluetooth, and augmented GPS signal strengths have been employed to gather this information. Until date, passive, receive-only satellite GPS sensing relied solely on signal strength and location information. This paper demonstrates that semi-processed GPS data (39 features) accessible to apps since Android 7 with precise location permissions can be used as a highly accurate leaky channel for sensing ambient, recognising human activity, and mapping indoor spaces (99%+ accuracy). This report describes a longitudinal research that used semi-processed GPS readings from mobile devices throughout a 40,000 sq. km region for a year. Data was acquired from aeroplanes, cruise ships, and high-altitude places. To retain crucial information, we analyse all satellite GPS signals and select the best characteristics using cross-correlation analysis. Our work, AndroCon, combines lin-ear discriminant analysis, unscented Kalman filtering, gradient boosting, and random forest learning to provide an accurate ambient and human activity sensor. At AndroCon, basic ML algorithms are used for discreet and somewhat explainable outcomes. We can readily recognise challenging situations, such as being in a subway, when someone is waving a hand in front of a mobile device, in front of a stairway, or with others present (not always carrying phones). This is the most extensive study on satellite GPS-based sensing as of yet.

==> removed.tex <==

\section {Exploring Raw GPS Data}
%\begin{figure}[htb]
%    \centering
%    \hspace{-2mm}
%    \includegraphics[width=0.5\textwidth]{images/raw.pdf}
%    \caption{Location API in Android 6 and Android 7}
%    \caption*{Source: https://www.euspa.europa.eu/newsroom/news/available-now-white-paper-using-gnss-raw-measurements-android-devices}
%    \label{fig:euspa}
%\end{figure}
%This includes the {android.location.GnssClock} API for obtaining measurements of the GNSS receiver’s clock, and the {android.location.GnssMeasurement} API for accessing raw GNSS measurements. 

%Tables~\ref{tab:gnssclock} and~\ref{tab:gnssmeasurement} summarize the variables present in the \texttt{GnssClock} and \texttt{GnssMeasurement}, respectively.
%\end{comment}

%The GnssMeasurement API values within the location package mirror the environmental characteristics of the user's location. Let us elaborate.

%FIXME: This should be there in the background (if this information is not there)
Raw GNSS observations were not accessible. 
Smartphone GNSS modules typically offered 3 to 5 meter accuracy in favorable multipath conditions but surpassed 10 meters in harsh multipath environments.  This limited accuracy prompted initiatives to enhance the precision of smartphone GNSS positioning.

\begin{comment}
    This section initially illustrates the correlation between GPS raw parameters and EM wave properties (see Figure~\ref{fig:mindmap}). Subsequently, we demonstrate the capability of this correlation in discerning the user's physical environment. The goal is to validate the existence of side-channel information.
\end{comment}

\begin{comment}
    In this section, we will demonstrate how various GnssMeasurement variables as illustrated in Table~\ref{tab:gnssmeasurement}, correlate with the user's physical environment. The objective is to establish the presence of side-channel information.
\end{comment}

\begin{comment}
\noindent{\textbf {\emph {\circled{2} PseudorangeRateUncertainity}}}:
This indicates the uncertainty in the pseudorangerate measurement, with its variability reflecting various scenarios and environmental conditions, akin to the pseudorangerate. In crowded or mobile environments, multipath effects and irregular Doppler measurements increase uncertainty, resulting in high PseudorangeRateUncertainity value. Conversely, in open areas, uncertainty decreases due to minimal multipath effects, leading to low PRRU values.
\end{comment}
\begin{comment}
    
\noindent{\textbf {\emph {\circled{3} ReceivedSvTimeUncertainty}}:
This parameter denotes the error estimate (1-$\sigma$) for the received GNSS time of a specific satellite vehicle. As it characterizes uncertainty, its efficacy in discerning user activity and ambiance mirrors PRU's.
\end{comment}

